Learning, Optimizing, and Simulating Fermions with Quantum Computers

Fermions are fundamental particles which obey seemingly bizarre quantum-mechanical principles, yet constitute all the ordinary matter that we inhabit. As such, their study is heavily motivated from both fundamental and practical incentives. In this dissertation, we will explore how the tools of quantum information and computation can assist us on both of these fronts. We primarily do so through the task of partial state learning: tomographic protocols for acquiring a reduced, but sufficient, classical description of a quantum system. Developing fast methods for partial tomography addresses a critical bottleneck in quantum simulation algorithms, which is a particularly pressing issue for currently available, imperfect quantum machines. At the same time, in the search for such protocols, we also refine our notion of what it means to learn quantum states. One important example is the ability to articulate, from a computational perspective, how the learning of fermions contrasts with other types of particles.

==> abstract.tex <==
% the abstract
\begin{doublespace}
Fermions are fundamental particles which obey seemingly bizarre quantum-mechanical principles, yet constitute all the ordinary matter that we inhabit. As such, their study is heavily motivated from both fundamental and practical incentives. In this dissertation, we will explore how the tools of quantum information and computation can assist us on both of these fronts. We primarily do so through the task of partial state learning:~tomographic protocols for acquiring a reduced, but sufficient, classical description of a quantum system. Developing fast methods for partial tomography addresses a critical bottleneck in quantum simulation algorithms, which is a particularly pressing issue for currently available, imperfect quantum machines. At the same time, in the search for such protocols, we also refine our notion of what it means to learn quantum states. One important example is the ability to articulate, from a computational perspective, how the learning of fermions contrasts with other types of particles.

The main results of this dissertation are as follows. First, we introduce a protocol called fermionic classical shadows that efficiently learns all local properties of a many-fermion system. We furthermore show that this protocol is optimal, in the sense that information-theoretic arguments imply matching lower bounds for the fundamental complexity of this learning task. Next, we extend the theory to a noise-robust formulation called symmetry-adjusted classical shadows, which uses symmetry in the quantum system to mitigate errors that occur during the quantum computation. We establish a rigorous theory for this protocol, as well as demonstrate realistic, near-term performance with comprehensive numerical experiments. We then study unitary partitioning, an alternative strategy for easing the measurement complexity of Hamiltonians for interacting electrons. Finally, we draw surprising connections between a hard classical optimization problem, known as the noncommutative Grothendieck problem, and the simulation of fermions. We establish a natural embedding of the classical problem into a fermionic one and provide both theoretical and numerical evidence that quantum computers can provide high-quality solutions over classical approximations through this embedding.
\end{doublespace}

% 150-word version
% This dissertation explores the application of quantum computers to the study of interacting fermions. We primarily tackle the problem of partial state learning:~protocols to efficiently acquire a reduced description of the quantum system. The first protocol we introduce, fermionic classical shadows, optimally learns all local properties of a many-fermion system. Next, we extend the theory to a noise-robust formulation called symmetry-adjusted classical shadows, which uses symmetry in the system to mitigate errors from the quantum computation. Such techniques are necessary for accurate simulations on currently available, noisy quantum machines. We also study unitary partitioning, an alternative protocol which eases the measurement complexity of interacting-electron Hamiltonians. Finally, we draw surprising connections between a hard classical optimization problem, the noncommutative Grothendieck problem, and the simulation of fermions. We establish an embedding of the classical problem into a fermionic one and demonstrate that quantum computers can provide high-quality solutions over classical approximations.

==> dedication.tex <==
% dedication text

To my family.


==> preface.tex <==
\epigraph{\emph{``A-A-R-G-H, numbers! Never mention numbers here. Only use them when we absolutely have to.''}}{\emph{The Phantom Tollbooth}\\\textsc{Norton Juster}}

==> thanks.tex <==
% the acknowledgments section

First and foremost, I thank my family for their continual support and unconditional love. My parents are at the core of everything that I have accomplished, and I would not be where I am without the foundation they have built for me. Likewise, my brothers have always been there for me, whether to inspire confidence in me or simply to make the daily passage of time more enjoyable. I am beyond fortunate to have my family at my back, not just during the course of this degree but throughout my life.

I am grateful to a number of mentors who have helped guide my descent into quantumness. At the forefront is my advisor, Akimasa Miyake, who instilled in me the makings of an effective researcher. His training stressed not only technical ability, but also the importance of soft skills such as communicating science at all levels of background. Akimasa entrusted me with considerable amounts of freedom and independence in my research goals, and I am thankful for his support over the entire course of my graduate career.

To the rest of my dissertation committee, I also give thanks:~Ivan Deutsch, whose infectious passion for physics has shaped how I approach science---not as a cold, analytical endeavor, but a wholly human one;~Milad Marvian, whose presence at CQuIC and breadth of expertise pushes the center to new frontiers;~and Andrew Landahl, whose unadulterated curiosity for all things physics and math reminds us why we continue to pursue science. Beyond my committee, Albuquerque has had no shortage of great people in quantum, and from both CQuIC and Sandia I would like to thank Elizabeth Crosson, Susan Atlas, Tameem Albash, Andrew Baczewski, and Ojas Parekh for the various subjects that they have taught me about. I would also like to thank my collaborators from Tufts---Peter Love, Andrew Tranter, and Will Kirby---who were instrumental in helping me put out my first paper.

I give special thanks to Shelby Kimmel, my earliest mentor in quantum. Shelby introduced me to the field while at Maryland, when I was a lost undergraduate who had just switched into physics. Through her mentorship I was able to experience not only research in quantum, but also as a theorist, an opportunity that I am truly grateful for. Shelby was also the one who recommended that I apply to UNM for my graduate studies;~without her guidance, this dissertation might never have been written.

No PhD student can make it without the support of their department, and I am no exception to that. First, thanks to my P{\&}A cohort:~Bryan, Pratik, Siva, Tyler, and Vikas. I really appreciated the tight-knit size of our class, as it gave us a special sense of camaraderie. Next, thanks to the Miyake group, both past and present---Adrian, Austin, Tyler, Vikas, Bruna, Ben, Cole, Alex, and Shravan---which has grown considerably since I started. And to everyone else who helped make this dissertation possible in one way or another, I thank you:~Changhao, Chaithanya, Sam, Mingyang, Manuel, Karthik, Anupam, Andrew, Spencer, Jake, Jalan, Jun, Lu, John, Philip, Marco, Raf, Pablo, and Chris. I also have immense gratitude to the administrative staff, namely Dwight Zier, Alisa Gibson, and Gloria Cordova, for enabling me to focus on my studies and research with minimal friction.

Finally, I would like to thank the quantum algorithms team at Google for their hospitality during my internship. That experience introduced me to unique and valuable ways of thinking about research that I would not have been exposed to at CQuIC alone. As I move into my future endeavors, I hope to bring some of that ethos along with me. I would especially like to highlight the small but plucky group at the San Francisco office---Nick Rubin, Bill Huggins, Fionn Malone, and Kianna Wan---with whom it was a pleasure to interact and learn from. Nick in particular has been a highly supportive mentor to me, encouraging me to seek bold directions and have confidence in the vision for my research. I owe many of my successes to his belief in my abilities and ideas.
